Sensorimotor Control Strategies for Tactile Robotics

How are robots becoming smarter at interacting with their surroundings? Recent advances have reshaped how robots use tactile sensing to perceive and engage with the world. Tactile sensing is a game-changer, allowing robots to embed sensorimotor control strategies to interact with complex environments and skillfully handle heterogeneous objects. Such control frameworks plan contact-driven motions while staying responsive to sudden changes. We review the latest methods for building perception and control systems in tactile robotics while offering practical guidelines for their design and implementation. We also address key challenges to shape the future of intelligent robots.

==> sections/misc.tex <==
% Sensors

A popular approach to face this complexity consists of building a world model based on a priori knowledge, and fusing sensory data to drive action selection. The so-called sensory-dependent task definition is an interesting alternative for adaptive robots \cite{hosoda2000}. According to this paradigm, the task is defined in the sensory space, which is the perceptual representation of the environment from sensors. Unlike the world model, which requires prior knowledge and calibration of the robot and the environment, the sensory space does not need any a priori information and can adapt to changes and uncertainties. The behavior is not hard-coded and results from the interaction with the world.
